Mining the Factor Zoo: Estimation of Latent Factor Models with Sufficient Proxies

Latent factor model estimation typically relies on either using domain knowledge to manually pick several observed covariates as factor proxies, or purely conducting multivariate analysis such as principal component analysis. However, the former approach may suffer from the bias while the latter can not incorporate additional information. We propose to bridge these two approaches while allowing the number of factor proxies to diverge, and hence make the latent factor model estimation robust, flexible, and statistically more accurate. As a bonus, the number of factors is also allowed to grow. At the heart of our method is a penalized reduced rank regression to combine information. To further deal with heavy-tailed data, a computationally attractive penalized robust reduced rank regression method is proposed. We establish faster rates of convergence compared with the benchmark. Extensive simulations and real examples are used to illustrate the advantages.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}


==> tables/tab1_old.tex <==
% \begin{table}[h]
% \centering
% \begin{tabular}{cccccccccccc}
%     \toprule
%     {} & {} & \multicolumn{5}{c}{Factors} & \multicolumn{5}{c}{Factors}\\
%     \cmidrule{1-12}
%     %  \cmidrule{5-5} 
%     $\omega_2$ & $\omega_1$ & PCA & PLS & PCR & SPCA & OP  & PCA  & PLS & PCR   & SPCA  & OP \\
%     \midrule
%     \multirow{2}{*}{0.7} & 1          &  0.69 & 0.56 & 0.979 & 0.639 & 0.201 & 0.612 & 0.511 & 0.982 & 0.66 & 0.403  \\
%     {}& 2          &  0.69 & 0.56 & 0.979 & 0.639 & 0.201 & 0.612 & 0.511 & 0.982 & 0.66 & 0.403  \\
%     \midrule
%     \multirow{2}{*}{0.7} & 1          &  0.69 & 0.56 & 0.979 & 0.639 & 0.201 & 0.612 & 0.511 & 0.982 & 0.66 & 0.403  \\
%     {}& 2          &  0.69 & 0.56 & 0.979 & 0.639 & 0.201 & 0.612 & 0.511 & 0.982 & 0.66 & 0.403  \\
%     \bottomrule
% \end{tabular}
% \end{table}



\begin{table}[h!]
\centering
\caption{Relative value of the smallest canonical correlations with FMSP as the denominator, when $\vec{g}(\vec{z}_t) = \vec{z}_t$ and under the \textit{i.i.d} setting. 
A value lower than 1 implies the estimation is less accurate than FMSP.}
\begin{tabular}{|c|c|ccccc|ccccc|}
\hline
                      &            & \multicolumn{5}{c|}{Factors} & \multicolumn{5}{c|}{Loading} \\ \hline
$\omega_2$            & $\omega_1$ &  PLS & PCR & PCA & SPCA & OP  & PLS & PCR & PCA & SPCA & OP \\ \hline
\multirow{3}{*}{0.7}   &  1  &  0.74 & 0.65 & 0.99 & 0.64 & 0.19 & 0.57 & 0.47 & 0.98 & 0.57 & 0.34 \\ 

 &  2  &  0.56 & 0.55 & 0.99 & 0.72 & 0.31 & 0.51 & 0.41 & 1.00 & 0.64 & 0.49 \\ 

 &  5  &  0.75 & 0.62 & 0.98 & 0.88 & 0.60 & 0.60 & 0.48 & 1.01 & 0.80 & 0.78 \\ 

\hline \multirow{3}{*}{0.95}
 &  1  &  1.11 & 0.99 & 0.72 & 0.65 & 0.32 & 0.91 & 0.83 & 0.78 & 0.63 & 0.51 \\ 

 &  2  &  0.68 & 0.62 & 0.81 & 0.79 & 0.57 & 0.66 & 0.61 & 0.85 & 0.74 & 0.74 \\ 

 &  5  &  0.86 & 0.72 & 0.79 & 0.98 & 0.95 & 0.81 & 0.64 & 0.86 & 0.98 & 1.05 \\ 
  \hline
\end{tabular}\label{tab:non_robust_IID}
\caption{Relative value of the smallest canonical correlations with FMSP as the denominator,  when $\vec{g}(\vec{z}_t) = 0.5 ( sin(\frac{1}{2}\vec{z}_t) +  \vec{z}_t)$ and under the \textit{i.i.d} setting. A value lower than 1 implies the estimation is less accurate than FMSP. }
\begin{tabular}{|c|c|ccccc|ccccc|}
\hline
                      &            & \multicolumn{5}{c|}{Factors} & \multicolumn{5}{c|}{Loading} \\ \hline
$\omega_2$            & $\omega_1$ & PLS & PCR & PCA & SPCA & OP  & PLS & PCR & PCA & SPCA & OP \\ \hline
\multirow{3}{*}{0.7}   &  1  &  0.61 & 0.52 & 0.99 & 0.62 & 0.21 & 0.48 & 0.44 & 1.02 & 0.56 & 0.34 \\ 

 &  2  &  0.54 & 0.52 & 1.00 & 0.67 & 0.30 & 0.46 & 0.40 & 1.01 & 0.57 & 0.42 \\ 

 &  5  &  0.65 & 0.57 & 1.01 & 0.81 & 0.50 & 0.53 & 0.46 & 1.01 & 0.70 & 0.65 \\ 

\hline \multirow{3}{*}{0.95}
 &  1  &  1.14 & 1.04 & 0.79 & 0.68 & 0.42 & 1.05 & 0.94 & 0.92 & 0.76 & 0.63 \\ 

 &  2  &  0.70 & 0.65 & 0.78 & 0.68 & 0.56 & 0.73 & 0.69 & 0.94 & 0.74 & 0.75 \\ 

 &  5  &  0.88 & 0.74 & 0.80 & 0.96 & 1.02 & 0.80 & 0.67 & 0.88 & 0.95 & 1.10 \\ 
                      \hline
\end{tabular}\label{tab:non_robust_sin_IID}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h!]
\centering
\caption{Relative value of the smallest canonical correlations with FMSP as the denominator, when $\vec{g}(\vec{z}_t) = \vec{z}_t$ and under the \textit{serial dependent} setting. 
A value lower than 1 implies the estimation is less accurate than FMSP.}
\begin{tabular}{|c|c|ccccc|ccccc|}
\hline
                      &            & \multicolumn{5}{c|}{Factors} & \multicolumn{5}{c|}{Loading} \\ \hline
$\omega_2$            & $\omega_1$ &  PLS & PCR & PCA & SPCA & OP  & PLS & PCR & PCA & SPCA & OP \\ \hline
\multirow{3}{*}{0.7}   &  1  &  0.72 & 0.59 & 1.00 & 0.69 & 0.21 & 0.59 & 0.49 & 1.00 & 0.58 & 0.38 \\ 

 &  2  &  0.64 & 0.57 & 0.99 & 0.79 & 0.35 & 0.53 & 0.44 & 1.00 & 0.70 & 0.54 \\ 

 &  5  &  0.71 & 0.62 & 0.99 & 0.93 & 0.68 & 0.57 & 0.44 & 1.00 & 0.85 & 0.84 \\ 

\hline \multirow{3}{*}{0.95}
 &  1  &  0.96 & 0.74 & 0.78 & 0.65 & 0.29 & 0.85 & 0.67 & 0.85 & 0.64 & 0.47 \\ 

 &  2  &  0.69 & 0.62 & 0.89 & 0.82 & 0.54 & 0.66 & 0.58 & 0.89 & 0.75 & 0.74 \\ 

 &  5  &  0.79 & 0.68 & 0.90 & 1.05 & 1.03 & 0.72 & 0.55 & 0.92 & 1.00 & 1.04 \\ 
\hline
\end{tabular}\label{tab:non_robust_TS}
\caption{Relative value of the smallest canonical correlations with FMSP as the denominator,  when $\vec{g}(\vec{z}_t) = 0.5 ( sin(\frac{1}{2}\vec{z}_t) +  \vec{z}_t)$ and under the \textit{serial dependent} setting. A value lower than 1 implies the estimation is less accurate than FMSP. }
\begin{tabular}{|c|c|ccccc|ccccc|}
\hline
                      &            & \multicolumn{5}{c|}{Factors} & \multicolumn{5}{c|}{Loading} \\ \hline
$\omega_2$            & $\omega_1$ & PLS & PCR & PCA & SPCA & OP  & PLS & PCR & PCA & SPCA & OP \\ \hline
\multirow{3}{*}{0.7}   &  1  &  0.61 & 0.54 & 1.00 & 0.57 & 0.19 & 0.51 & 0.43 & 1.02 & 0.54 & 0.33 \\ 

 &  2  &  0.63 & 0.52 & 1.01 & 0.68 & 0.31 & 0.49 & 0.41 & 1.00 & 0.59 & 0.49 \\ 

 &  5  &  0.61 & 0.56 & 1.00 & 0.86 & 0.57 & 0.55 & 0.41 & 1.01 & 0.76 & 0.73 \\ 

\hline \multirow{3}{*}{0.95}
 &  1  &  0.99 & 0.80 & 0.80 & 0.62 & 0.37 & 0.88 & 0.72 & 0.89 & 0.62 & 0.57 \\ 

 &  2  &  0.78 & 0.69 & 0.89 & 0.79 & 0.61 & 0.72 & 0.62 & 0.90 & 0.72 & 0.75 \\ 

 &  5  &  0.81 & 0.71 & 0.89 & 1.05 & 1.06 & 0.74 & 0.61 & 0.93 & 1.00 & 1.07 \\ 
                      \hline
\end{tabular}\label{tab:non_robust_sin_TS}
\end{table}

